PowerCut and Obfuscator: An Exploration of the Design Space for Privacy-Preserving Interventions for Voice Assistants

The pervasive use of smart speakers has raised numerous privacy concerns. While work to date provides an understanding of user perceptions of these threats, limited research focuses on how we can mitigate these concerns, either through redesigning the smart speaker or through dedicated privacy-preserving interventions. In this paper, we present the design and prototyping of two privacy-preserving interventions: `Obfuscator' targeted at disabling recording at the microphones, and `PowerCut' targeted at disabling power to the smart speaker. We present our findings from a technology probe study involving 24 households that interacted with our prototypes; the primary objective was to gain a better understanding of the design space for technological interventions that might address these concerns. Our data and findings reveal complex trade-offs among utility, privacy, and usability and stresses the importance of multi-functionality, aesthetics, ease-of-use, and form factor. We discuss the implications of our findings for the development of subsequent interventions and the future design of smart speakers.

==> Contents/Unused/00_title.tex <==
%   \author*[1]{Corresponding Author}

%   \author[2]{Second Author}

%   \author[3]{Third Author}

%   \author[4]{Fourth Author}

%   \affil[1]{Affil, E-mail: email@email.edu}

%   \affil[2]{Affil, E-mail: email@email.edu}

%   \affil[3]{Affil, E-mail: email@email.edu}

%   \affil[4]{Affil, E-mail: email@email.edu}
  
 \title{Blackout and Obfuscator: An Exploration of the Design Space for \\ Privacy-Preserving Interventions for Smart Speakers}
%   \runningtitle{Blackout and Obfuscator: An Exploration of the Design Space for Privacy-Preserving Interventions for Smart Speakers}
  
  
\input{Contents/0_abstract.tex}
\maketitle

==> Contents/Unused/z5_results_orig.tex <==
\section{Observations}
\label{sec:findings}

%\textcolor{blue}{PENDING: should i remove the take-aways from this section?}

\begin{table}[t]
\small
\label{table:themes}
\begin{center}
\begin{tabular}{ p{8cm}}
\toprule
{\bf Attitudes towards Smart Speaker} \\ 
\midrule
Characterizes the user's (a) nature and awareness, (b) technological know-how, (c) trust in \va manufacturer, and (d) perceptions towards listening and recording. \\ %\hline
\toprule
{\bf Attitudes towards Intervention}\\ 
\midrule
Characterizes the user's (a) interaction preference, (b) comfort-levels with regards to usage, (c) long-term technological preferences, and (d) trust attitude towards intervention. \\ %\hline
\toprule
{\bf Aesthetics and Physical Footprint}\\ 
\midrule
Characterizes the user's (a) aesthetics preference, (b) physical footprint preference, (c) perception of the informativeness of cues, and (d) preference between bolt-on and built-in interventions.\\ %\hline
\toprule
{\bf Utility of Interventions}\\ 
\midrule
Characterizes the user's preference with respect to intervention's (a) multifunctionality, (b) cost, (c) ability to provide fine-grained control, and (d) mode of operation \ie proactive vs. reactive,  \\ %\hline
\bottomrule
\end{tabular}
\end{center}
\caption{Summary of the extracted themes.}
\label{themes}
\end{table}

In this section, we discuss the four key themes that emerged from our analysis. In summary, we found that: 1. Participants were reluctant in sacrificing the convenience associated with \vas; hands-free interaction was most preferred, and physical interaction was seen as being not ideal; 2. Participants expected bolt-on interventions with existing household decor and to offer cues informing them of the state of both the intervention and the \va; 3. Multifunctionality, fine-grained control (per-user and per-device), and cost of the intervention are important factors that might influence adoption; 4. While participants believed in both active and passive privacy violations, they were comfortable with their conversations being overheard because they believed that their conversations were not sensitive (in comparison to information available using their location/web footprint).


% \subsection{Privacy Perceptions}

% Our pre- and post- interaction surveys aimed to establish the privacy baseline and how this baseline changed after the interview. While we acknowledge that more detailed and longer studies were required to accurately estimate participants' privacy preferences, we believe that our questionnaires serve as a coarse proxy. 

% \textcolor{red}{VC: remove quotes about child beating}


\subsection{User Attitudes regarding Smart Speakers}

\noindent{\em 1. Types of Users:} Through our study, we identified two types of users: (a) {\em casual users} who utilize their \vas for setting alarms, asking questions etc., and (b) {\em power users} who have integrated the \vas with other devices in their homes (such as smart lights, house monitoring systems etc.). We also observed that most participants in our first interview phase were casual users, and a majority of those in the second phase were power users. This phenomena could be based on the pervasive availability and easy installation of various smart home devices. We observed that power users were also more familiar with passive privacy violations and with the potential for active violations (though not the specifics of how this may occur). Consistent with our expectations, we observed that users in the second interview phase were aware of recent privacy violations. We expect that power users will be more willing to adapt privacy-preserving interventions as they have more to lose if their devices were compromised, \ie as their households were more tightly integrated with the \va. We also observed that a majority of the participants did not change their conversations around the \vas (in comparison to conversations in rooms without \vas), but a small minority reported feeling conscious of having discussion around them.\\
%\textbf{Takeaway:} Despite participant familiarity with \va technology, there are gaps in their understanding of how privacy violations manifest themselves. This suggests promise in designing interventions for the same.

%\vspace{1mm}
\noindent{\em 2. Understanding of \va operation:} We observed that a minority of the participants were unaware of how \va's operate, \ie they were unaware that their vocal commands were processed off-site. Participant $P_5$, for example, believed that the \vas did \textit{``some local learning but also some more... I think at some point people were involved in [the processing]... I think there's an automated learning that occurs to adjust itself to the household right?''}  These perceptions were shared across participants with different educational backgrounds. \\

%\sout{\textbf{Takeaway:} Despite participant familiarity with \va technology, there are gaps in their understanding of how \va functionality. This suggests that interventions designed must be easy to understand.}

%\vspace{1mm}
\noindent{\em 3. Trust in device manufacturers:} Trust in the device manufacturers fragmented our participant population. This includes fractions (a) that believed that these organizations can be trusted; their belief comes from faith in the legal system which would penalize organizations if there is evidence indicating malpractice, (b) that believed that some manufacturers were not in the business of collecting personal information and can be trusted, (c) that trusted the manufacturers, but believed that any information collected could be leaked, or shared with other organizations they do not trust, and (d) that trusted the manufacturers as long as there is personal utility from their information being collected. A recurrent theme was participants' comfort in being recorded because they believed they were part of a large pool of \va users, and their vocal footprint provided corporations no additional insight into their lives. Participant $P_{10}$ explains, \textit{``I mean we're not planning any nefarious capers... like we're very boring people and therefore nothing that we're talking about would be of interest to anyone on the other end of [the \va].''} Some participants justified this notion by commenting on the nature of advertisements they received after introducing the \va in their homes; $P_8$ states \textit{``the way Google that Google ads operates ... you know if... I talk about something; it starts showing up ... if I'm scrolling through Facebook.''} \\{\bf Takeaway:} The participants' trust in the device manufacturer is mixed, which benefits third party developers.

%\vspace{1mm}

%\textcolor{blue}{PENDING: This doesn't seem to be related to the solution design in anyway, so can we scrap it all?}
%\sout{\noindent{\em 4. Vocal footprint vs. other sources of information:} Some participants suggested that the {\em vocal footprint} shared with \vas is both limited and not as informative as their web footprint and location information. Participant $P_2$ states, ``my information is certainly more out there on social media than it is [with \vas]. I also I don't feel like I have anything to hide... I mean if they use my information it's going to be for some monetary reason like to sell to me.'' These participants also believed that social engineering is a more potent form of harm than audio-based profiling. Participants' perceptions did not conform to academic attack models. While we observed that participants were comfortable if their conversations were overheard, they were uncomfortable if the entity overhearing is a human \ie participants were more comfortable with algorithms digesting their information. However, all participants agreed that {\em storing} data was unacceptable.\\
%{\bf Takeaway:} Participants believe that vocal information contains lesser context, and is not as informative as other information they share over the internet. This can primarily be attributed to the lack of widespread media attention given to how vocal information can be misused, suggesting that privacy is a reactive requirement. }

\subsection{User Attitudes regarding the Probes}

\noindent{\em 1. State of operation:}
Participants believed that the current designs of the probes make it too inconvenient to use the \va. They state that using them  makes the interaction with a \va a two-phase procedure: first check the state of the probe (engaged vs. not) and disengage if necessary, and then interact with the \va. They claim that the additional set of steps defeats the purpose of owning a \va \xspace \ie to have spontaneous interactions. Some participants stated that the probes added a {\em mental burden} in terms of remembering its state. Participant $P_9$ said: {\em ``when you were to power it off say how do you distinguish that state [when it has no power when using \boutT] from a wake word doing nothing, like I don't know I unmute this right now ... it looks the same.''} However, participants believed that owning these probes will serve as a contingency if there is documented evidence of foul play; $P_9$ states \textit{``we lock our doors at night; it's [the] proactive step... nothing bad might happen... it's insurance pretty much.''}\\ %We already know from earlier research~\cite{Machuletz:2018} that the user's choice to deploy privacy-enhancing technologies in the physical world is influenced by passive control over privacy more than initial concerns about privacy.
%\sout{{\bf Takeaway:} Participants prefer to be aware of the state of the intervention (on vs. off) at all times; interventions that require additional interaction to determine the state are not preferred.}  

%\vspace{1mm}
\noindent{\em 2. Ergonomics:} Participants were comfortable with the {\em usability} of the probes. They were easy to set up and use, and the time taken for the probes to get engaged is acceptable (almost instantaneous in all cases). However, participants expressed dissatisfaction at the longer boot-up times induced by \boutT. For example, $P_8$ stated,\textit{``I would find it especially irritating.''} Participants suggested that technologies such as \obfT that, when disengaged, make the \va immediately available were ideal; $P_{13}$ explains, \textit{``I'd probably lean more towards something like [the \obfT] over even like just the outlet for the convenience factor of like you can turn that off with a button and not really have to worry about [the Dot] like warming up.''} Some participants were concerned about the generalizability of \obfT. They believed that the technology is specific to their \vas, and would not extend to future \vas or \vas made by other vendors. Participants were also comfortable with the interventions because they were not connected to the internet (and thus believed that the \obfT intervention will not be a privacy violation). Their comfort levels with the interventions were tied to their belief that manufacturer heterogeneity introduces greater privacy protection, \ie neither \boutT nor \obfT were manufactured by the \va manufacturers. In fact, participant $P_{10}$, when asked if they had a preference over the intervention developer, replied: \textit{``I wouldn't but I'm sure like older generations would feel much more comfortable ... if it came from McAfee.''}

We observed that participants unanimously found the mute-button the least convenient; the act of walking to the \va to (dis-)engage imposed a significant usability barrier. Participants were more comfortable using a remote control, but felt that their homes have many remotes, and that the remotes could be easily misplaced. When proposing the addition of another remote, $P_5$ exclaimed, \textit{``they're all over the place, so many remotes! We can't have another remote.''} Some participants suggested moving intervention control to a mobile phone app; unlike remote controls, participants believed that their mobile phones were less prone to being misplaced and alleviate other issues pertaining to remotes. Finally, participants were apprehensive in imagining a voice-controlled intervention (as they were informed of how \vas currently process voice commands off-site).\\ %We assuaged their apprehensions by hypothesizing voice commands that could be processed locally; we will discuss this in more detail in \textcolor{red}{design section}.
%\sout{{\bf Takeaway:} Ease of interaction (remote/vocal vs. physical) is a key discriminating factor. Smart speakers are preferred due to their hands-free interaction system, and interventions that operate in a similar manner are ideal.}

%\vspace{1mm}
\noindent{\em 3. Trust in bolt-on interventions:} Finally, participants trust our bolt-on probes more than the built-in mute button. Participants suggested that trust in the bolt-on intervention would be low if it came from the device manufacturer, or any organization that had a similar business model. Participant $P_{13}$ recommended \textit{``a competing company or just a general company that seems like they're like honest''} could develop the interventions. Participants suggested that bolt-on interventions were easier to debug, and were easier to understand. However, participants feel that purchasing one bolt-on intervention for every \va is not economically feasible.\\

%\sout{{\bf Takeaway:} The business model of third-party developers should be different from that of the \va manufacturers. This enhances user trust.} 

\subsection{Aesthetics \& Physical Footprint}

With regards to the mute button, participants felt comfortable with its design and placement, while finding it inconvenient to use. A very small fraction of the participants were unaware of the existence of the mute button or its utility.

\begin{figure}
 \centering
  \includegraphics[width=\columnwidth]{Images/owl-alexa.png}
  \caption{The placement of an Amazon Echo Dot inside an owl-shaped holder in one of the households.\vspace*{-6mm}}
  \label{fig:placement}
\end{figure} 

\noindent{\em 1. Physical Footprint:} Participants were concerned with the physical footprint of our probes. While \vas were electronic devices, participants often associate them with decorative items (Figure~\ref{fig:placement}) and invest effort in determining where these devices should be placed. A common example of a description about the \obfT solution we received was $P_2$'s description: \textit{``a piling on of devices.''}  Some participants found it difficult to reorganize other items around the \va to facilitate the probe. Additionally, some participants prefer to conceal their outlets, and \boutT-like interventions were inconvenient in such scenarios. Participants were uncomfortable with interventions that involve additional wires (as in the case of \obfT). \\

%\sout{{\bf Takeaway:} The intervention must not be larger than the \va, and must not necessitate reorganizing existing decor.}

%\vspace{1mm}
%\sout{\textcolor{blue}{PENDING: related to the earlier "state of operation" point? }
%\noindent{\em 2. Cues:} Another point of contention is the utility of visual cues in the interventions. Recall that \boutT has an LED indicator that glows red when engaged; participants found the the color of the indicator a red herring --- the red color led participants to believe that the device was malfunctioning. This situation is further exacerbated in the scenario where participants preferred to have their outlets hidden. Participants did not notice that the probes had visual cues, and believed that this complicated understanding its state (on vs. off). While participants found the visual cues uninformative in some settings, they did state that having cues relieves burdens associated with ascertaining device/intervention state. They suggested that other cues, which should be more informative, would be preferred in such situations. For example, $P_9$ states that they would like to \textit{"see the video [of the \obfT signal] feedback to the [listening] device, but have [the \obfT haptic light] go green when it's working}."\\
%{\bf Takeaway:} As suggested earlier, participants prefer informative (and intuitive) cues provided by the interventions.} 

%\vspace{1mm}

%\textcolor{blue}{PENDING: contradicts earlier point on trust in bolt-on solutions? }

%\sout{\noindent{\em 3. Preference towards built-in solutions:} Few participants suggested that they would prefer a {\em trustworthy built-in} intervention; this could be designed as software updates (or skills) that could be added to the \va. They argue that built-in interventions were preferred as they do not add to the physical footprint of the \va, and it does not add additional economic strain. Building upon what was discussed earlier, participants suggested that their ideal built-in intervention should also be voice activated. While participants do not trust the device manufacturer, they are willing to trust the in-built privacy provision they provide, ergo contradicting themselves. \\%How one can design such an intervention, potentially using techniques from cryptography and secure hardware design, is out of the scope of this paper. \\
%{\bf Takeaway:} Ease-of-use dictates adoption; participants fail to see the contradiction when they state preference of built-in solutions from manufacturers they do not trust. }


\subsection{Utility of the Interventions}

\noindent{\em 1. Damage to environment:} Participants were concerned that \obfT will cause harm to animals present in their homes; questions we received upon presenting the \obfT were often like $P_2$'s, \textit{``is [this] going to ... make my dog crazy?''} While we did not observe any agitation/discomfort, the participants suggested that their pets could perceive the ultrasound signals, and were not bothered by it. Additionally, participants were concerned about exposing their \vas to ultrasound for a prolonged period of time\footnote{A detailed study is needed to understand the impact of ultrasound on electronic devices.}.\\ 
%{\bf Takeaway:} Interventions must not cause damage to the surrounding ecosystem. Proof of the same is ideal.

%\vspace{1mm}
\noindent{\em 2. Cost and Multi-Functionality:} Cost was repeatedly discussed; participants suggested that the cost of the interventions should not exceed the cost of the \va. Some participants received their \vas as gifts, and were unaware of their market value. Consequently, they were unable to establish a value for the intervention; $P_6$ states, \textit{``that's a really interesting question in the sense that I didn't pay for this in the first place. Maybe that's also another reason that I don't have much investment in using this in general.''} On the other end of the investment spectrum, we observed that participants who owned multiple smart devices were invested in safeguarding their privacy, and were willing to adopt the interventions independent of the cost. Participant $P_6$, who had previously stopped using their \vas due to privacy concern, even stated that they would consider using their device once more given that the intervention were, \textit{``cheap... I think would have to rival that remote plug-in cost right because ... it has to be like a cheap utility ... or a cheap accessory like that.''} Participants were concerned about the amount of electricity consumed by \obfT; \obfT could be used in a proactive way \ie always-on, or in a reactive way \ie use when needed. Participants felt that a reactive approach, though tedious, would be easier to understand. Participants also believed that a (potentially high) cost could be justified if the intervention provided multiple features. This could be achieved by integrating the design of \obfT with other home decor, such as lamps, lights, clocks, radios. \\
%{\bf Takeaway:} Customizable (and affordable) interventions are more preferred. Aesthetic preferences vary, and there is no aesthetic design that suits all participants. 

%\vspace{1mm}
\noindent{\em 3. Fine-Grained Control:} The final observation we make is an extension to multi-functionality; we observed that in some households, some participants preferred to utilize the intervention more than others. In such scenarios, they desired customized usage profiles based on their requirements \ie \xspace {\em fine-grained control per-user}. Another observation we make is that some participants preferred to have one intervention (like \obfT) being used to preserve privacy against a wide range of \va-like devices. In such scenarios, {\em fine-grained control per-device} was desired. Based on the current design of the \obfT prototype, meeting both these requirements is challenging, and requires further research. \\
%{\bf Takeaway:} Multi-user, multi-preference interventions are preferred to static interventions.
%\textcolor{red}{note on customized control per-user vs per-device}



==> Contents/Unused/z6_discussion.tex <==
\section{Design Implications}
\label{design}

% expand significantly; make two pages

% 1. aesthetics: personalizable; integrate with home decor
% 2. ease of deployment + understanding
% 3. cost
% 4. trusted technology
% 5. physical size
% 6. provide more than one feature
% 7. customizable for each person in the household
% 8. hands-free
% 9. informative cue
% 10. “ideally in-built” with the \va --> kassem, judge if this is needed here.
% 11. immediate availability when not under intervention's control --> pending


% We stress that these findings are not ordered to reflect their importance. We also stress that these findings are useful for redesigning \vas factoring in privacy for users.
\begin{table}[h!]
\small
%\label{table:designs}
\begin{center}
\begin{tabular}{ p{8.1cm}}
\toprule
{\bf 1. Aesthetics} \\ 
\midrule
The interventions should be offered in different forms, shapes, and colors to fit within people decors and furniture.
 \\ %\hline
\toprule
{\bf 2. Physical Footprint}\\ 
\midrule
The footprint of the intervention should be small enough to not force a reorganization of the layout of owner's house. \\ %\hline
\toprule
{\bf 3. Multi-Functionality}\\ 
\midrule
The intervention is better when providing additional functionality (such as a clock) to reduce its footprint and integrate better with home decor. \\ %\hline
\toprule
{\bf 4. Ease of Deployment and Understanding}\\ 
\midrule
Battery-powered interventions  are easier to deploy. Also, proper understanding of the privacy metaphor improves the adoption of interventions. \\ %\hline
\toprule
{\bf 5. Trust in Technology}\\ 
\midrule
Trustworthy interventions are: bolt-on, not network connected, designed by a different trustworthy organization, and pose no additional risk. \\ %\hline
\toprule
{\bf 6. Mode of Interaction}\\ 
\midrule
Using the intervention should not change the interaction with the \va. Hands-free interaction is most preferable. %with the intervention, possibly using voice activation, is more preferable. 
\\ %\hline
\toprule
{\bf 7. Informative Cues}\\ 
\midrule
Interventions should offer cues that communicate their state. Visual, auditory, or text cues might be applicable depending on the deployment. \\ %\hline
\toprule
{\bf 8. Cost}\\ 
\midrule
The intervention should cost less than the \va. \\ %\hline
\toprule
{\bf 9. Fine-grained Privacy Control}\\ 
\midrule
The intervention can offer per-user and per-\va privacy controls.  \\ %\hline
\toprule
{\bf 10. Awareness}\\ 
\midrule
Awareness of privacy violations increases trust in intervention designers.  \\ %\hline
\bottomrule
\end{tabular}
\end{center}
\caption{Summary of the identified design guidelines. \textcolor{red}{VC: do we need this table?}}
%\vspace*{-6mm}
\label{findings}
\end{table}


In our observations and analysis, several themes emerged which offer the following implications (Table~\ref{findings}) for the design of privacy-preserving interventions for \vas. 

\textcolor{red}{VC: for each theme -- provide a "design recommendation" i.e. a brief one or two liner on what we think the design should be; should also discuss scenarios where the intervention can be used + how it will be used}


\vspace{1mm}
\noindent{\em 1. Aesthetics:} We observed the aesthetics of the privacy interventions to be an important issue for our participants. While they appreciated the value provided by both \boutT and \obfT, participants felt uncomfortable with their current designs. Even though \obfT's current design (as opposed to earlier versions) seemed more homespun, participants preferred the interventions to match their individual decorating styles (one example is shown in Figure~\ref{fig:placement}). Many participants suggested that the intervention should come in different forms, shapes, and colors, enabling easier integration within their home decor. As individual tastes vary widely, devising a one-fits-all design is challenging. One possible approach is to explore different design options for different types of users, including shapes, forms, colors, and material. This approach has been successful with \vas, where participants feel comfortable with the aesthetic of the \va. For example, Amazon has four offerings of their Echo product featuring combinations of forms and fabric colors. With time, participants perceived the \va's design to become more polished, from an inexpensive plastic exterior, to more refined design (with fabric and different colors). Participants expressed similar concerns about \boutT, but stressed more upon its physical footprint, which we discuss next.

\textcolor{red}{VC: homespun + variety of colors + fabrics; also add that it should not be harmful to animals}


\vspace{1mm}
\noindent{\em 2. Physical Footprint:} Since the \vas we considered were small and compact, participants preferred a similar physical footprint for the interventions. Several participants expressed concerns regarding the size of both \boutT and \obfT, suggesting that similar functionality could be achieved with a smaller prototype. They believed that using \obfT (which also needs to be placed close to the \va) requires them to significantly reorganize their existing layout. We discuss how this requirement can be mitigated in the next paragraph about {\em Multi-Functionality}. While the form factor of \boutT can be reduced trivially, doing so for \obfT requires additional research; the size and shape of the horn speaker in our current prototype was chosen to ensure maximum ultrasound distribution and coverage. Extending such a design to \vas that are larger, or have a different orientation for the microphone inputs will require rethinking the design and form factor.

\textcolor{red}{VC: small + can be concealable}


\vspace{1mm}
\noindent{\em 3. Multi-Functionality:} Closely tied to the aesthetics, participants indicated preference toward an intervention (specifically \obfT) that offered features beyond privacy-preservation. They suggested that the \obfT intervention could be combined with other household artifacts, such as a lamp, radio, clock etc. Doing so reduces the footprint of the intervention. Multi-functionality provides an alternative avenue for customizing the product, making it easier to integrate with existing household decoration. Participants who are worried about the social stigma of being labeled as overly privacy-conscious would benefit from such designs, \ie, the intervention would be inconspicuous. Another interpretation of this point could be to envision interventions as artifacts that co-exist with the \va, such as a stand to hold the \va,\footnote{\url{https://www.amazon.com/Speaker-Stand-Amazon-Other-Models/dp/B01K1O7UFM}}, or a sleeve for the \va.\footnote{\url{https://www.amazon.com/PINE-PAINT-LLC-Unicorn-Speaker/dp/B07V3TCQ7R/ref=sr_1_3?keywords=decorative+holders+for+alexa&qid=1568402536&s=amazon-devices&sr=8-3}} There is a demand for such artifacts based on our analysis of reviews for such products, and we believe such designs would promote adoption.

\textcolor{red}{VC: should also provide additional functionality; best would be a container for the device}


\vspace{1mm}
\noindent{\em 4. Ease of Deployment and Understanding:} Participants preferred to have a solution that was easy to deploy in their homes; the biggest impediment to any intervention similar to \boutT is its physical footprint. Many participants preferred to conceal the interventions' wiring, and the nearby outlets can be hard to reach. Attaching \boutT to wall outlets, even once, requires considerable re-positioning of other devices and their wires. Attaching \obfT would require an additional outlet, which is not always readily available. One na\"ive solution would be to split the outlet among multiple devices. Participants suggested that an \obfT design capable of operating on batteries would be more preferred, even if this required periodic replacement. Participants also suggested that since the current version of an \obfT-style intervention will not operate in an {\em always-on} mode, the energy consumption will be limited. All participants were able to easily grasp the metaphor associated with \boutT, but the technology behind \obfT proved complicated for some. Thus, interventions whose operation is easy to explain may be preferred. While \obfT is easy to use once deployed, debugging it may pose problems for users who are lack proper understanding of its operation. We also believe that understanding the detriments (if any) of ultrasound towards humans, animals, and other electronics may put users at ease.
% \footnote{Based on our current analysis, there are none.}.

%kassem: something related to the above, we can design \obf to share the same wiring as the va. for example, the intervention could be connected to the usb outlet of the va, and the intervention is wall-powered. (intervention means obfuscator in this case).--> added something along these lines

\textcolor{red}{VC: provide a tutorial of some sort as part of the installation}


\vspace{1mm}
\noindent{\em 5. Trust in the Technology:} Participants were more comfortable with technologies that they believe will survive the ``test of time,'' \ie, be useful for \va models in the future. The privacy guarantees of \boutT can be thwarted by \vas that are battery operated. However, thwarting \obfT's guarantees is more challenging and would potentially require much more expensive microphones. As discussed earlier, trust also stems from knowing that the interventions do not pose any additional risk. Specifically, we observed that (a) participants wanted to know about any detriments introduced by the interventions such as potential damage to the \va by frequently disconnecting it from its power source or subjecting it to ultrasound; and (b) our current interventions are not network connected and do not present the same risks as the \vas. Finally, participants preferred our bolt-on interventions as opposed to the built-in interventions as they were designed by an organization they trusted (more than the \va manufacturers). 

\textcolor{red}{VC: third party is preferred; especially from academic institutions}


\vspace{1mm}
\noindent{\em 6. Mode of Interaction:} We observed that participants placed a high value on the {\em convenience} of using \vas from which they are not willing to compromise. Thus, interventions that, when disengaged, delay the \va operation (as in the case of \boutT) are not preferred (even though \boutT provably preserves privacy, and its mode of operation is very easy to understand). Additionally, any form of physical interaction, be it using remotes or buttons, is far from ideal; some participants expressed preference toward using an app on their smartphones. We believe that future privacy-preserving solutions must be designed so as to disrupt the convenience of the use of these systems minimally. An ideal design would have a voice interface that allows the user to control it as they control their \vas. However, such an always-on and listening privacy-preserving solution can have the same pitfalls as \vas, and they must be designed in a manner that does not erode user trust. For example, the can lack a network interface to provide the users with hard privacy assurances. Another issue that may arise with voice-activated interventions is erroneous activations; understanding how this can be minimized requires additional research. 
 
\textcolor{red}{VC: hands-free is preferred (ideal) but has its own issues; remote + app is less preferred; not connected to internet = ideal}
 
 %%%%modify this slightly 
\vspace{1mm}
\noindent{\em 7. Informative Cues:} As stated earlier, some participants concealed their \vas and would prefer concealing their interventions as well. Some participants take this notion to the extreme; they believe that any electronic device that does not provide extensive visual information should be concealed. Thus, visual cues are not ideal in all situations. Additionally, participants suggested that the {\em red} light on the \boutT intervention suggested that the intervention was broken, as opposed to indicating the state of the intervention. Interacting with the \va when the intervention is enabled helps users determine the state of the \va (operational vs. not), but such an approach is reactive. Participants indicated preference for a {\em proactive} approach. Combined with the observation that visual cues are not informative, we believe that auditory cues may be preferable. The \obfT-style intervention can announce using speech or text that the \va is inactive when users try to activate it.
 
\textcolor{red}{VC: should always know the state of operation}

%  Alternatively, the intervention can inform users of the state of the device through text (using Bluetooth-based protocols).
 

\vspace{1mm}
\noindent{\em 8. Cost:} Another factor that impacts adoption is cost of the \va. A large fraction of our participants own smart plugs similar to \boutT, leading us to believe that such an intervention is affordable. However, the cost of prototyping \obfT was \$70, exceeding the cost of \vas (priced at approx. \$30). This cost includes the price of the commodity parts needed to construct the prototype. Participants believe that the cost of the intervention should not exceed the cost of the \va; this is especially true if the intervention can provide privacy-protection against a single \va. We believe that if such an intervention would be adopted widely, the production costs could be amortized. Additionally, understanding the engineering requirements to design an \obfT-like intervention that provides privacy against various \vas located at different parts of a home requires independent research. 

\textcolor{red}{VC: should be cheap}


\vspace{1mm}
\noindent{\em 9. Fine-grained Privacy Control:} Several households owned more than a single \va, and they had members with different (and potentially conflicting) privacy requirements. Thus, we believe that there is a requirement for (a) fine-grained control \textit{per user} and (b) fine-grained control \textit{per \va}. For the latter, a na\"ive solution would be to deploy one intervention for every \va in the household, but depending on the cost per intervention, such a solution may not scale. Thus, an ideal design would provide privacy protection for more than one \va. This design could be conceptualized as smaller interventions co-located with the \vas but controlled centrally. Providing per-user control is a more challenging problem; it requires understanding how disparate the privacy requirements are, how frequently users are utilizing a \va together, and how to mitigate conflicts should they arise. Providing a solution to this problem requires additional research~\cite{zeng2019understanding}.


\vspace{1mm}
\noindent{\em 10. Effect of Awareness:} Based on our pre- and post-interview questionnaires, we observed the following trend amidst the participants of our interview phases. The participants of our second phase are more concerned about the potential privacy threats from the \vas (in comparison to the participants of the first phase, who are also concerned). This concern stems from increased awareness; recent \va mishaps, erroneous code used in them, and immoral practices by device manufacturers have led to an increasing concern amidst the participants. Based on our discussion, we observed that participants believe that these issues are not being seriously audited by the device manufacturers. Discussing various loopholes that can be implemented in the built-in interventions in the status quo (\ie local wake word processing, and the mute button) also increased participants' awareness. Due to these factors, participants believe that interventions created by third parties (who do not share the same business motives as the device manufacturer) provide the desired privacy properties. 




==> Contents/Unused/z6_discussion_copy.tex <==
\section{Design Implications}
\label{design}

% expand significantly; make two pages

% 1. aesthetics: personalizable; integrate with home decor
% 2. ease of deployment + understanding
% 3. cost
% 4. trusted technology
% 5. physical size
% 6. provide more than one feature
% 7. customizable for each person in the household
% 8. hands-free
% 9. informative cue
% 10. “ideally in-built” with the \va --> kassem, judge if this is needed here.

Through our analysis and results reported in earlier sections, several themes emerged which can inform both \va and privacy-preserving intervention design. We highlight these below. We stress that these findings are not ordered to reflect their importance.

{\em 1. Aesthetics:} Aesthetics of objects and devices at home is an extensively studied topic~\cite{}. Aesthetics of interventions is no different. While users appreciated the value provided by them, they were uncomfortable with their (both \boutT and \obfT) current designs. While \obfT's current design (as opposed to earlier versions) seemed more homespun, it did not resonate with participants who preferred something more "unique" to their individual styles. Many participants suggested that the aesthetic should resemble home decor, while numerous options should be provided to make them customizable. Realizing these requirements is a challenging proposition; user tastes vary widely, and coming up with a design that suits all, or options for various types of users is challenging, and worth follow up research. Participants expressed similar concerns about \boutT, but stressed upon its physical footprint, which we discuss next.

{\em 2. Physical Footprint:} Since the \vas we considered were small and compact, participants preferred a similar physical footprint for the interventions. Several participants expressed concerns regarding the size of both \boutT and \obfT, suggesting that similar functionality could be achieved with a smaller prototype. While the form factor of \boutT can be reduced trivially, doing so for \obfT requires additional research; the size and shape of the horn speaker in our current prototype was chosen to ensure maximum ultrasound distribution and coverage. 

{\em 3. Ease of Deployment and Understanding:} Participants preferred to have a solution that was easy to deploy in their homes; the biggest impediment to any intervention similar to \boutT is its physical footprint. Many participants preferred to conceal their wiring, and the corresponding outlets are hard to reach. Attaching such an intervention, even once, requires considerable re-positioning of other devices. Participants suggest that an \obfT design capable of operating on batteries would be more preferred, even if this required periodic replacement. Participants claim that since the \obfT-style intervention won't operate in an {\em always-on} mode, the energy consumption will be limited. All participants were able to easily grasp the metaphor associated with \boutT, but the technology behind \obfT proved complicated for some. Thus, interventions whose operation is easy to explain seem to be preferred more. While \obfT is easy to use once deployed, debugging it may pose problems for users who are unaware of its operation; such an observation is not new and exists in prior works~\cite{}.

{\em 4. Trust in the Technology:} Closely tied to the earlier point, participants are more comfortable with technologies they believe will survive the "test of time" \ie be useful for \va releases in the future. The privacy guarantees of \boutT can be thwarted by \vas that are battery operated. However, thwarting \obfT's guarantees is more challenging (and would potentially require expensive beam-forming capabilities). While we did not discuss this point with our participants in great detail, we believe it is valuable; most research in the security and privacy community considers an {\em adaptive} adversary model.

{\em 5. Mode of Interaction:} We observed that participants place a high value on the {\em convenience} of using \vas from which they are not willing to compromise; any form of physical interaction, (be it using remotes or buttons) are far from the ideal, though some participants prefer to use an app on their smartphones. We believe that future privacy-preserving solutions must be designed so as to disrupt the convenience of the use of these systems minimally. An ideal design should have a voice interface that allows the user to control it as they control their \vas. However, such an always-on, listening privacy-preserving solution can have the same pitfalls as \vas, and they must be designed in a manner that does not erode user trust, for example, by lacking a network interface to provide the users with hard privacy assurances.

{\em 6. Cost:} Another factor that impacts adoption is cost of the \va. A large fraction of our participants own smart plugs similar to \bouT, leading us to believe that such an intervention is affordable. However, the cost of prototyping \obfT was \$ \textcolor{red}{kassem: 2000202}, exceeding the cost of \vas (priced at approx. \$ 30). Participants believe that the cost of the intervention should not exceed the cost of the \va; this is especially true if the intervention can provide privacy-protection from a single \va. Understanding the engineering requirements to design an \obfT-like intervention that provides privacy against various \vas located at different parts of a home requires independent research. 

{\em 7. Multi-Functionality:} Closely tied to the aesthetics, participants indicated preference towards an intervention that offered features beyond privacy-preservation. They suggested that the \obfT intervention could be combined with other household artifacts, such as a lamp, radio, vase, clock etc. This provides an alternative avenue for customizing the product, making it easy to integrate with households. Additionally, participants who are worried of being labeled privacy-conscious would benefit from such designs. Another interpretation of this point could be to envision interventions as artifacts that co-exist with the \va, such as a stand to hold the \va \footnote{http://tiny.cc/v7jpcz}, or a sleeve for the \va \footnote{http://tiny.cc/16jpcz}. 

{\em 8. Informative Cues:} As stated earlier, some participants conceal their devices. Thus, visual cues are not ideal in all situations. Additionally, participants suggested that the {\em red} light on the \boutT intervention suggested that the intervention was broken, as opposed to indicating the state of the intervention. Interacting with the \va when the intervention is enabled helps users determine the state of the \va (operational vs. not), but such an approach is reactive. Participants indicated preference for a {\em proactive} approach. Combined with the observation that visual cues are not informative, we believe that auditory cues may be ideal. The \obfT-style intervention can periodically announce that the \va is inactive. Alternatively, the intervention can inform users of the state of the device through text (using Bluetooth-based protocols).

==> title.tex <==
\title{Blackout and Obfuscator: An Exploration of the Design Space for Privacy-Preserving Interventions for \vas}
\def\plainauthor{Author name(s) for PDF metadata. Don't forget to anonymize for submission!}
\author{Varun Chandrasekaran, Kassem Fawaz, Bilge Mutlu, Suman Banerjee \\ University of Wisconsin-Madison \\ \{chandrasekaran, kfawaz, bilge, suman\}@cs.wisc.edu}

\pagestyle{plain}

